Expect More from the Networking: DDoS Mitigation by FITT in Named Data Networking

Distributed Denial of Service (DDoS) attacks have plagued the Internet for decades, but the basic defense approaches have not fundamentally changed. Rather, the size and rate of growth in attacks have actually outpaced carriers' and DDoS mitigation services' growth, calling for new solutions that can be, partially or fully, deployed imminently and exhibit effectiveness. In this paper, we examine the basic functions in Named Data Networking (NDN), a newly proposed Internet architecture, that can address the principle weaknesses in today's IP networks. We demonstrate by a new DDoS mitigation solution over NDN, Fine-grained Interest Traffic Throttling FITT, that NDN's architectural changes, even when incrementally deployed, can make DDoS attacks fundamentally more difficult to launch and less effective. FITT leverages the NDN design to enable the network to detect DDoS from victim's feedback, throttles DDoS traffic by reverse its exact paths through the network, and enforces control over the misbehaving entities at their sources. Our extensive simulation results show that FITT can throttle attack traffic with one-way time delay from the victim to the NDN gateway; upon activation, FITT effectively stop attack traffic from impacting benign flows, resulting in over 99\% of packets reaching victims being legitimate ones. We further demonstrate that service providers may implement NDN/FITT on existing CDN nodes as an incrementally deployable solution to effectuate the application level remediation at the sources, which remains unattainable in today's DDoS mitigation approaches.

==> sections/deploy.tex <==
\section{Incremental Deployment of \sysname}
\label{sec:deploy}

\todo{Remove the whole section with some content go to other sections.}

%% To enable \sysname to combat DDoS threats thanks to today's IoT market, in this section, we present the mechanism for service providers to incrementally deploy \sysname onto the existing IoT network and devices.
%% It is not required for the whole network infrastructure to run NDN.
%% With service providers being able to own both ends of the communications (e.g., mobile devices and IoT network gateways), one could take a page out of Google's QUIC~\cite{quic-sigcomm17} and migrate both ends of the communications from the current network stack to NDN-based network stack and \sysname.
%% Between the two ends, service providers can deploy overlay NDN routers; the easiest and most efficient way of realizing this is to have edge network gateways (e.g., smart home gateway routers, edge computing severs) equipped with NDN stack.
%% \TODO{Add more.}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.35\textwidth]{figures/deploy}
	\caption{An Example Topology}
	\label{fig:deploy}
\end{figure}

%% We argue that even incremental deployment will help mitigate the DDoS attack for the following reasons.
%% \begin{itemize} [leftmargin=*, itemsep=1pt, parsep=2pt, topsep=4pt]
	%% \item Since millions of IoT devices have already been deployed and in use, if a service is getting buried by DDoS from the botnet like Mirai, there would be a strong motivation for it and other services to embrace NDN to eliminate their attack surface.
	%% \item With the overlay NDN routers and two ends speacking NDN, it is enough for \sysname to effectuate the DDoS mitigation. As shown in Figure~\ref{fig:deploy}, \TODO{Add more}.
%% \end{itemize}
%%
%% \subsection{Heterogeneous Networking}
%%
%% Similar to how QUIC and how IPv6 are being deployed, after NDN and \sysname being deployed partially, the legacy network and the NDN network will coexists.
%% To handle compatibility, the service provider can adopt the same strategy as QUIC does by simply using a fallback-to-IP mechanism in the handshake process.
%%
%%
%% \TODO{EO: I'll merge the above with this asap, this is just my first cut...}

% Incr depl is well served by aligning costs w/ incetives.


==> sections/discussion.tex <==
%\section{Discussion}
%\label{sec:discussion}
%
%\subsection{Authenticity of Victim's \sysname NACK}
%
%


==> sections/ip.tex <==
\section{DDoS Mitigation over TCP/IP Architecture}
%% \label{sec:related}
\label{sec:ip}

\angelos{Can go directly after intro.}

\angelos{Add discussion of blackhold and ddos scrubbing. And go earlier (like in intro)}

\subsection{DDoS and Vulnerabilities in IP}
%\TODO{Jan17 Call: : objective and matter-of-fact way: DDoS and IP's properties, not attacking.\\
%	Zhiyi: text revised.}
%
%\TODO{EO: I would tone this down and focus the descriptions to be a little more accurate.  
%The largest DDoS attacks capitaalize on source address spoofing (I would limit the claims to that), and TCP
%SYN attacks come in different flavors too (resource starvation, volumetric, etc.).  Reflective amplification attacks
%have large variances in the TTPs and combatting them is often done by application-level remediation (in scubbing systems, appliances, app configs, etc.)}

%% <EO> I think the below is redundant with what we should position in the intro... (I suggest) commenting out
% Many of the largest volumetric DDoS attacks that we have seen today have been maed possible by architectural properties that exist in TCP/IP.
% For example, the Mirai botnet was used to generate (then) unprecedented DDoS traffic volume, costing millions of dollars (in losses and mitigation service costs).
% In part, this resulted from the large numbers of sources that are still relatively easy to compromise: 
% IP address enumeration and scanning trivialize the
% discovery of poorly protected IoT devices, which can then be used to build the biggest botnet ever.
% Another example is that reflective amplification attacks capitalize on source address spoofing and redirect traffic to any IP addresses~\cite{mirai-botnet}.  
% DDoS attacks have large variances in their TTPs and combating them is often done by application-level remediation (in scrubbing systems, appliances, app configurations, etc.)




%congestion control in the current TCP/IP architecture cannot help to mitigate DDoS for the following reasons:
% \TODO{Lixia:this should relate to later mentioning about push back: that requires hop-by-hop state about the traffic: \\
% Therefore, there is no real enforcement and thus attackers can freely violate the congestion control.
% Current congestion control exists at the transport layer but not all transport layer protocols have implemented congestion control, e.g., UDP.
% }

% Based on these observations of IP networking, \cite{handley04-steps,off-by-default} propose modifications to the existing Internet architecture to have greater DDoS resilience at an architectural level.
% A number of desired features of a DDoS-resistant Internet architecture are presented, the major ones include 


%% \subsection{Network-centric DDoS Mitigation}
%% %There have been various solutions constructed around defending DDoS attacks.
%% %Following the taxonomy defined in the previous works~\cite{DDoStaxonomy, geva2014bandwidth}, we take several representative approaches as examples and analyze how those mechanisms work but are limited by the nature of IP networking. 
%% 
%% Deployable filter-based network-level remediation approaches in TCP/IP like FlowSpec~\cite{RFC5575}, RTBH~\cite{RFC5635}, the IETF's Distributed Open Threat Signaling (dots) Working Group~\cite{ietf-dots} etc., lack the necessary expressiveness of DDoS's TTPs. 
%% Such mechanisms would additionally require Deep Packet Inspection (DPI) to gain insight into the ongoing traffic which IP's stateless forwarding cannot provide.
%% For instance, black-hole filtering blacklists entire network prefixes, which can cause collateral damage to: well-behaved sources, non-attack traffic that is sourced from compromised devices, etc.
%% As another example, FlowSpec requires the proper n-tuple consisting of several matching criteria so that DDoS traffic can be classified; however, since most supported matching criteria is at the network layer (e.g., IPv4, IPv6, ICMP), FlowSpec can mistakenly drop legitimate traffic to other services deployed on the same victim server or block good traffic sent from the compromised bots.
%% 
%% Ioannidis and Bellovin proposed router-based Pushback~\cite{ioannidis2002pushback} which utilizes a heuristics function to detect packets that \emph{probably} belong to an attacker by checking the ``congestion signature'' (e.g., source/destination addresses) of the traffic.
%% Due to routers' coarse-grained inspection of traffic, the filtering can lead to collateral damage.
%% 
%% Another interesting work is Active Internet Traffic Filtering (AITF)~\cite{argyraki2005active}, which requires the routers on the path of attacking traffic to mark traffic flows with route records (RRs), which are the IP addresses of routers who have forwarded the flow.
%% In this way, the victim can report the unexpected flows to the network, and routers can filter the flows identified by the RRs.
%% However, this may potentially cause damage to 
%% \begin{enumerate*} [label=(\roman*)]
%% 	\item all the traffic (both attack traffic and legitimate) sent along the path, because RRs cannot distinguish application-level flows,
%% 	and
%% 	\item legitimate hosts who are under the same first hop network as the attackers, because routers do not have fine-grain state to identify exact senders.
%% \end{enumerate*}
%% %In addition, deployment of these approaches would require updating routing infrastructure in core Internet Service Provider (ISP) routers, without incentives for those ISPs to undertake such an upgrade.
%% 
%% Some other network-based works like StopIt~\cite{liu2008filter} and SIFF~\cite{yaar2004siff} require additional features that are missing in the existing TCP/IP architecture.
%% For example, SIFF introduces privileged communication, which requires additional information carried by the IP header and each router on the connection path marking IP packets.
%% %Filter-based and rate limiting approaches such as Ingress Filtering~\cite{RFC2827}, Pushback~\cite{ioannidis2002pushback}, Remote Triggered Back-Holing (RTBH)~\cite{RFC5635} and some other recent works~\cite{liu2008filter, yaar2004siff} utilize detection mechanisms to identify offending traffic and control the traffic by filtering it out or applying rate limiting.
%% %These mechanisms require Deep Packet Inspection (DPI) to have an insight into the ongoing traffic.
%% %However, the forwarding in IP routers lacks the state of the traffic; for example, the IP forwarder cannot distinguish the flows from different applications without additional overhead.
%% %Thus, these mechanisms take the risk of causing collateral damage on the legitimate traffic.
%% Capability-based approaches like TVA (Traffic Validation Architecture)~\cite{xiaowei05-dos-limiting, liu2008passport} introduce authentication of the packet source into the network system. 
%% Taking TVA as an example, by embedding cryptographic authentication info into the IP packet, the routing system and servers are able to distinguish legitimate users from ``bad'' ones.
%% The primary difficulties in operationally deploying these proposed solutions are adding extra functionality into the deployed TCP/IP architecture
%% and an incentive misalignment similar to Pushback.
%% 
%% %Ioannidis and Bellovin proposed a realization of router-based Pushback~\cite{ioannidis2002pushback} based on IP networking. 
%% %To overcome the difficulty of knowing with certainty whether a packet actually belongs to a "good" or a "bad" flow, their proposed solution utilizes a heuristics function to detect packets that \emph{probably} belong to an attacker. 
%% %This is done by using the ``congestion signature".
%% %Routers can thus preferentially drop the packets.
%% %However, it is hard to implement this Pushback defense, due to the difficulty of getting the congestion signature and the lack of forwarding insights provided by the routers.
%% 
%% %Compared with \cite{ioannidis2002pushback}, our approach based on NDN utilizes the victim's feedback and the traffic states provided by NDN at each router would help the system know with certainty the source of the overwhelming traffic.
%% %Ultimately, our proposed Pushback learns which clients are not obeying the DDoS control and has the ability to selectively rate limit only those clients. 
%% %% <EO> I don't know if we want to broach this, but it is part of our story...
%% % Additionally, these approaches (Pushback, TVA, etc.) lack an incentive model for incremental deployment.
%% </EO>


==> sections/rational.tex <==



%\section{\sysname Protection Methods}
%
%% From the design description, we can see \sysname directly makes use of NDN's properties to combat DDoS:
%\sysname directly makes use of NDN's properties to combat DDoS in the following ways:
%\begin{itemize} [leftmargin=*, itemsep=1pt, parsep=2pt, topsep=4pt]
%	\item Utilizing structured names at the network layer allows \sysname to perform service-level, per-prefix, reaction and monitoring.
%	\item Stateful forwarding provides exact information about the traffic so that \sysname can accurately identify suspicious clients.
%  \item Remediating traffic at sources alleviates network congestion and capacity concerns of data producers and intermediate network infrastructure (like Internet eXchange Points, IXPs, etc.).
%\end{itemize}
%
%\subsection{Victim's Feedback enables Accuracy}
%
%%\TODO{EO: I don't think the below text should remain.  Section sec:ndn:previous (as it is currently written) does not talk about the item for IP DDoS, and I feel the statements are a little misleading.}
%%Starting DDoS countermeasures by routers' detection of the underlying traffic poses a risk of denying services to good clients.
%%Usually, such detection requires pre-configured threshold values as discussed in Section~\ref{sec:ndn:previous}.
%%Moreover, routers need to learn about the server capacities in advance so that defense mechanisms will not control the traffic too strictly (no traffic to the server at all) or too loosely (permitted traffic still overwhelms the server).
%%Therefore, in the \sysname system, we let the victim server be responsible for detecting a DDoS attack and sending \sysname NACKs downstream to trigger Pushback.
%%Thus, our system does not require any pre-configured thresholds in routers.
%
%The explicit feedback enables \sysname to perform fine-grained DDoS mitigation.
%To be specific, the prefix $PREF$ helps \sysname narrow the target traffic scope and the capacity $C$ can inform the downstream routers about the percentage volume of traffic that should be controlled in case of valid Interest (I-1 or I-3) overwhelm.
%Moreover, hearing the feedback also makes the reaction more accurate: NACK's $RSN$ helps routers to learn the attack type and take different actions accordingly.
%In case of fake Interest attacks, by tracking the incoming interfaces of the Interests listed in $FakeList$, routers are able to directly identify the attackers and completely block them.
%
%
%%Another benefit of \sysname is that the routers don't need to maintain any additional information if there is no reported DDoS attack from servers; all actions in \sysname are triggered only after a \sysname NACK from the victim is received.
%
%Since the design is built to mitigate DDoS for a variety of prefixes and types of Interest Attacks, \sysname is able to handle complex scenarios.
%For example, more than one victim server can send multiple NACKs containing different prefixes and different reasons.
%
%
%\subsection{Minimizing Collateral Damage by Fine Granularity}
%
%
%
%\subsection{Distributed Throttling at Sources}
%
%In our design, only \sysname edge routers play the role of rate limiting.
%This is because, on one hand, we cannot trust a client's device to take actions - it could be compromised as well.
%On the other hand, an upstream router should not perform rate limiting for the following reasons:
%\begin{enumerate*} [label=(\roman*)]
%\item When the traffic volume under a target prefix increases, upstream routers do not have enough knowledge to tell whether it is because of the misbehaving downstream routers or new clients have joined.
%\item When legitimate clients are behind a downstream router, compared with edge routers, upstream router actions will also hurt legitimate clients.
%\end{enumerate*}
%Note that this is one reason why attempts to remediate DDoS in IP networks (using FlowSpec, RTBH, etc.) suffer and are often maligned, because of the collateral damage that can result from their use.
%
%In cases when an edge router is connected to downstream routers or clients that are not equipped with NDN and \sysname, our proposed approach still reduces the attack surface by reinforcing the limitation on the suspect traffic.
%Because \sysname may cause collateral damage to the legitimate clients behind the edge routers (since clients can not be reached in this case) \sysname uses best-effort to mitigate the DDoS traffic to the victim.
%
%%% \TODO{EO: I would add some text in here that discusses the reduced attack surface that results when clients can't be reached (if they don't have named data) and the gateway is not necessarily directly attached to the devices either (even additional attack surface reduction).}
%
%\subsection{Monitoring Further Identifies Attackers}
%\label{sec:choices:cg}
%
%%After an edge router sends out NACKs to suspicious clients, we believe that the legitimate clients will obey the DDoS control and lower their sending rate of Interests accordingly while attackers may not abide by this.
%
%
%In valid Interest attack scenarios, a router calculates the weight by simply equally distributing the capacity among all suspect
%%\TODO{EO: First use of ``faces''?  Should this be defined earlier?}
%interfaces by equation~\ref{equation:valid}, which may potentially cause unfair capacity assignment to clients.
%For example,  $C1$ and $C2$ in Figure~\ref{fig:toy} will be assigned more capacity than $C3$ and $C4$ in a valid Interest attack reaction because $C1$ and $C2$ are closer to the victim in the topology, thus having larger weight.
%Though there is potential for unfairness, .
%
%%\TODO{Zhiyi: add how reinforcement throttling can correct the wrong weight assignments made by the routers.}
%%\TODO{Vishrant: Do we still need this? Any limits imposed on legitimate client will be lifted after timer resets and wrong weight assignment then wont have any 'bad' effects as they only work towards bad guys}
%
%%Since each router starts the limit at a different time because of the various round-trip time (RTT) between the victim server and each client gateway router, even though an attacker can reset its sending rate after the router removes the limit, there are no longer bursts of traffic and the attack becomes less harmful.

